Beyond the heat: The mental health toll of temperature and humidity in India

Evidence on the heat-mental health nexus remains mixed. I show that this can be partly explained by previous studies focusing solely on temperature while neglecting temperature-humidity interactions. Using a measure that considers both indicators (wet bulb temperature), I assess the causal link between extreme heat and mental health, and its heterogeneity across socioeconomic indicators. I combine self-reported depression and anxiety levels from three Indian WHO-SAGE survey waves with climate data, leveraging quasi-random variation in heat exposure due to survey timing and location. The results reveal that extreme heat increases the risk of depression but not of anxiety. Importantly, these effects are consistently smaller when humidity is not considered. Finally, the study provides evidence that the District Mental Health Program plays a protective role in mitigating adverse mental health effects. The findings suggest that the costs induced by climate change need to account for the economic consequences of deteriorated mental health.

==> Table3.tex <==

\begin{table}[h!]
	\caption{\label{gender}Gender heterogeneity}
	\centering
	\small
	\begin{tabular}{p{4.3cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}}
				\midrule
		\midrule
		& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
		& (1)                  & (2)                  & (3)                  & (4)                  & (5)                  & (6)                  \\
		& \multicolumn{3}{c}{\textbf{Men}}                                            & \multicolumn{3}{c}{\textbf{Women}}                                          \\
		& Depression           & Worry/ Anxiety        & Overall Happiness    & Depression           & Worry/ Anxiety        & Overall Happiness    \\
				\midrule
		&                      &                      &                      &                      &                      &                      \\
		Days $\geq$ 97.5\textsuperscript{th}  & 0.017***             & 0.020***             & 0.020***             & 0.016***             & 0.018***             & 0.022***             \\
	perc.	& (0.004)              & (0.005)              & (0.004)              & (0.004)              & (0.005)              & (0.003)              \\
		Heat wave (=1, $\geq$    & 0.144***             & 0.188***             & 0.153***             & 0.115***             & 0.113**              & 0.174***             \\
 3 days $\geq$ 97.5\textsuperscript{th} perc.) 		& (0.040)              & (0.047)              & (0.034)              & (0.037)              & (0.047)              & (0.027)              \\
		&                      &                      &                      &                      &                      &                      \\
		Observations        & 8,260                & 8,245             & 8,246                & 11,496               & 11,465               & 11,477               \\
		Weather Controls    &  \Checkmark                    &  \Checkmark                    &  \Checkmark                   &  \Checkmark                    &  \Checkmark                 & \Checkmark                   \\
		Year \& Week FE    &  \Checkmark                   &  \Checkmark                    &  \Checkmark                  &  \Checkmark                    &  \Checkmark                   &  \Checkmark                   \\
		KGC FE              &  \Checkmark                   &  \Checkmark                    &  \Checkmark                    &  \Checkmark                    &  \Checkmark                   &  \Checkmark                   \\
		\# of PSU           & 371                  & 371                  & 371                  & 371                  & 371                  & 371                  \\
		Mean               & 1.74 & 1.97 & 2.50 & 1.87 & 2.13 & 2.48 \\
	 P-value men=women (days) & 0.854 & 0.648 & 0.654 & & & \\
	  P-value men=women (bin.) & 0.435 & 0.072 & 0.477 & & & \\
		\midrule
		\midrule
		\multicolumn{7}{p{17.5cm}}{\textit{Notes:} Each coefficient stems from a separate regression in which the main explanatory variable is the variable indicated in the left column. Robust standard  errors are clustered at the PSU level and presented in parentheses. ***   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1}
\end{tabular}
\end{table}






\begin{table}[h!]
	\caption{\label{location}Urban-rural heterogeneity}
	\centering
	\small
		\begin{tabular}{p{4.3cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}C{1.75cm}}
		\midrule
		\midrule
		& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
		& (1)                  & (2)                  & (3)                  & (4)                  & (5)                  & (6)                  \\
		& \multicolumn{3}{c}{\textbf{Urban}}                                            & \multicolumn{3}{c}{\textbf{Rural}}                                          \\
		& Depression           & Worry/ Anxiety        & Overall Happiness    & Depression           & Worry/ Anxiety        & Overall Happiness    \\
		\midrule
		&                      &                      &                      &                      &                      &                      \\
		Days $\geq$ 97.5\textsuperscript{th} & 0.013**                   & 0.013                     & 0.020***                  & 0.021***                  & 0.023***                  & 0.022***                  \\
perc.	& (0.006)                   & (0.009)                   & (0.006)                   & (0.004)                   & (0.005)                   & (0.003)                   \\
     	Heat wave (=1, $\geq$                         & 0.100*                   & 0.083                     & 0.103**                   & 0.165***                  & 0.184***                  & 0.202***                  \\
 3 days $\geq$ 97.5\textsuperscript{th} perc.)	& (0.052)                   & (0.072)                   & (0.043)                   & (0.043)                   & (0.051)                   & (0.031)                   \\
	&                           &                           &                           &                           &                           &                           \\
	Observations                                           & 4,617                    & 4,609                     & 4,609                     & 15,139                   & 15,101                   & 15,114                    \\
		Weather Controls    &  \Checkmark                    &  \Checkmark                    &  \Checkmark                   &  \Checkmark                    &  \Checkmark                 & \Checkmark                   \\
		Year \& Week FE    &  \Checkmark                   &  \Checkmark                    &  \Checkmark                  &  \Checkmark                    &  \Checkmark                   &  \Checkmark                   \\
		KGC FE              &  \Checkmark                   &  \Checkmark                    &  \Checkmark                    &  \Checkmark                    &  \Checkmark                   &  \Checkmark                   \\
		\# of PSU           & 89                  & 89                 & 89              & 282                  & 282                  & 282                  \\
		Mean               & 1.67 & 1.87 & 2.34 & 1.85 & 2.12 & 2.53 \\
			 P-value urb.=rur. (days) & 0.245 & 0.343 & 0.752 & & & \\
		P-value urb.=rur. (bin.) & 0.332 & 0.251 & 0.060 & & & \\
		\midrule
		\midrule
		\multicolumn{7}{p{17.5cm}}{\textit{Notes:} Each coefficient stems from a separate regression in which the main explanatory variable is the variable indicated in the left column. Robust standard  errors are clustered at the PSU level and presented in parentheses. ***   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1}
	\end{tabular}
\end{table}

==> Table6_7.tex <==

	\begin{table}[h!]
		\caption{\label{channels_urban}Conflicts with others as channel}
		\centering
		\small
\begin{tabular}{p{3cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}}
	\midrule
	\midrule
	& (1)                    & (2)                    & (3)                       & (4)                      & (5)                   & (6)                   & (7)                      & (8)                      \\
	& \multicolumn{4}{c}{\textbf{Urban}}                                                                              & \multicolumn{4}{c}{\textbf{Rural}}                                                                           \\                              
	& \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II}
	\\                		& Conflict & Depression     & Conflict     & Depression   & Conflict     & Depression     & Conflict             & Depression           \\
	\midrule
		&               &                &              &                &              &                &                      &                      \\
		Conflicts                                  &               & 0.265***       &              & 0.265***       &              & 0.312***       &                      & 0.313***             \\
		&               & (0.020)        &              & (0.019)        &              & (0.011)        &                      & (0.011)              \\
		Days $\geq$ 97.5\textsuperscript{th} perc.      & 0.040***      & 0.002          &              &                & 0.040***     & 0.009***       &                      &                      \\
		& (0.008)       & (0.006)        &              &                & (0.005)      & (0.003)        &                      &                      \\
		Heat wave (=1)                                                    &               &                & 0.273***     & 0.028          &              &                & 0.334***             & 0.060            \\
		&               &                & (0.068)      & (0.047)        &              &                & (0.057)              & (0.038)              \\
		&               &                &              &                &              &                &                      &                      \\
\midrule
Direct effect & & 0.008 & & 0.028 & & 0.031*** & & 0.060
\\
Indirect effect & & 0.038*** & & 0.072*** & & 0.044*** & & 0.105**
\\
Total effect & & 0.046*** & & 0.100* & & 0.076***  & & 0.165***
\\
\midrule

Observations                                                      & 4,620         & 4,620          & 4,620        & 4,620          & 15,142       & 15,142         & 15,142               & 15,142               \\
Controls \& FE                                                    & \Checkmark                    & \Checkmark                    & \Checkmark                       & \Checkmark                      & \Checkmark                   & \Checkmark                   & \Checkmark                      & \Checkmark                      \\
		\# of PSU                                                         & 89            & 89             & 89           & 89             & 282          & 282            & 282                  & 282                  \\
		\midrule 
		\midrule 
		\multicolumn{9}{p{17cm}}{Standard errors are clustered at the PSU level and presented in parentheses. ***   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1.} 
	\end{tabular}
\end{table}



\begin{table}[h!]
	\caption{\label{channels_urban2}Sleeping problems as channel}
	\centering
	\small
	\begin{tabular}{p{3cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}C{1.3cm}C{1.4cm}}
		\midrule
		\midrule
		
		& (1)                    & (2)                    & (3)                       & (4)                      & (5)                   & (6)                   & (7)                      & (8)                      \\
		& \multicolumn{4}{c}{\textbf{Urban}}                                                                              & \multicolumn{4}{c}{\textbf{Rural}}  
		                                                                         \\    
	& \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II} & \textbf{I} & \textbf{II} \\                                          		& Sleeping  & Depression     & Sleeping      & Depression   & Sleeping      & Depression     & Sleeping              & Depression           \\
		& problems & & problems & & problems & & problems & \\
		\midrule
		&               &                &              &                &              &                &                      &                      \\
		Sleeping problems                                 &          & 0.431*** &          & 0.431*** &          & 0.442*** &          & 0.443*** \\
		&          & (0.020)  &          & (0.020)  &          & (0.010)  &          & (0.010)  \\
		Days $\geq$ 97.5\textsuperscript{th}   perc & 0.013** & 0.007   &          &          & 0.016*** & 0.014*** &          &          \\
		& (0.006)  & (0.005)  &          &          & (0.004)  & (0.003)  &          &          \\
		Heat wave (=1)                                               &          &          & 0.103** & 0.056   &          &          & 0.134*** & 0.106*** \\
		&          &          & (0.045)  & (0.046)  &          &          & (0.037)  & (0.034) \\
		&               &                &              &                &              &                &                      &                      \\
\midrule
Direct effect & & 0.025 &  &  0.056 & & 0.051*** & & 0.106***
\\
Indirect effect & & 0.020** & & 0.044** & & 0.025*** & & 0.060***
\\
Total effect & & 0.046** &  & 0.100* & & 0.076*** & & 0.165***
\\
\midrule
		Observations                                                      & 4,620         & 4,620          & 4,620        & 4,620          & 15,142       & 15,142         & 15,142               & 15,142               \\
	Controls \& FE                                                    & \Checkmark                    & \Checkmark                    & \Checkmark                       & \Checkmark                      & \Checkmark                   & \Checkmark                   & \Checkmark                      & \Checkmark                      \\
		\# of PSU                                                         & 89            & 89             & 89           & 89             & 282          & 282            & 282                  & 282                  \\
		\midrule 
		\midrule 
		\multicolumn{9}{p{17cm}}{Standard errors are clustered at the PSU level and presented in parentheses. ***   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1.} 
	\end{tabular}
\end{table}
